Impacts of magnetic permeability on electromagnetic data collected in settings with steel-cased wells

Electromagnetic methods are increasingly being applied in settings with steel infrastructure. These include applications such as monitoring of CO2 sequestration or even assessing the integrity of a wellbore. In this paper, we examine the impacts of the magnetic permeability of a steel-cased well on electromagnetic responses in grounded source experiments. We consider a vertical wellbore and simulate time and frequency domain data on 3D cylindrical meshes. Permeability slows the decay of surface electric fields in the time domain and contributes to a phase shift in the frequency domain. We develop our understanding of how permeability alters currents within, and external to, the casing by focussing first on the time domain response and translating insights to the frequency domain. Following others, we rewrite Maxwell's equations to separate the response into terms that describe the magnetization and induction effects. Magnetic permeability impacts the responses in two ways: (1) it enhances the inductive component of the response in the casing, and (2) it creates a magnetization current on the outer wall of the casing. The interaction of these two effects results in a poloidal current system within the casing. It also generates anomalous currents external to the casing that can alter the geometry and magnitude of currents in the surrounding geologic formation. This has the potential to be advantageous for enhancing responses in monitoring applications.

==> equations/faraday-freq.tex <==
\begin{equation}
\nabla \times \vec{E} = -i\omega\vec{B}
\label{eq:faraday-freq}
\end{equation}


==> equations/faraday-time.tex <==
\begin{equation}
\nabla \times \vec{e} = -\frac{\partial \vec{b}}{\partial t}
\label{eq:faraday-time}
\end{equation}


==> equations/permeability-ampere-no-source-freq-dc.tex <==
\begin{equation}
\nabla \times \vec{B} = \nabla \ln \mu_r \times \vec{B} + \mu\sigma\vec{E}
\label{eq:permeability-ampere-no-source-freq-dc}
\end{equation}


==> equations/permeability-derivation.tex <==
\begin{displaymath}
    \begin{split}
    \nabla \times \vec{h} - \vec{j} &= \vec{j}_s \\
    \nabla \times \frac{1}{\mu} \vec{b} - \vec{j} &= \vec{j}_s \\
    \frac{1}{\mu} \nabla \times \vec{b} + \left(\nabla \frac{1}{\mu}\right) \times \vec{b} - \vec{j} &= \vec{j}_s
    \end{split}
\label{eq:permeability-derivation}
\end{displaymath}


==> equations/reverse-triangle.tex <==
\begin{displaymath}
    \left|\vec{a} - \vec{b}\right| \geq \left| |\vec{a}| - |\vec{b}| \right|
\label{eq:reverse-triangle}
\end{displaymath}


==> figures/casing_flux_geometry.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=0.3\textwidth]{figures/casing_flux_geometry.png}
    \end{center}
\caption{
    Sketch of the geometry of the dominant geometry of the current density,
    $\vec{j}$ and magnetic flux density, $\vec{b}$, within the casing.
    Most of the current flows vertically
    while most of the magnetic flux density is rotational.
}
\label{fig:casing_flux_geometry}
\end{figure}





==> figures/current-systems-sketch.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=0.75\textwidth]{figures/current-systems-sketch.png}
    \end{center}
\caption{
    Sketch of the plan-view geometry of the early-time galvanic currents (left) and image currents (right) in a time-domain EM experiment over a half-space.
    Through time, both current systems diffuse downwards and outwards as they decay.
    The wire follows a straight line between the negative and positive electrodes. The green dashed line shows where we are measuring the
    radial electric field data. Prior to shut-off, current in the wire flows from
    the negative to the positive electrode. In the earth, the galvanic currents are dipolar in nature and flow
    from the positive to the negative electrode. Along the survey-line, the radial component of the galvanic currents always points outwards.
    Immediately after shut-off, image currents are induced in the earth. They are oriented in the same direction as the original current in the wire
    and are directed away from the negative electrode towards the positive. Along the survey-line, the radial component of the image currents is always pointed inwards.
}
\label{fig:current-systems-sketch}
\end{figure}





==> figures/excitation-time.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=\textwidth]{figures/excitation-time.png}
    \end{center}
\caption{
    Amplitude of the average electric field over a test volume that extends from 50m - 100m radially and 50m vertically centered about depths of (a) 100m and (e) 400m. The different line-styles in (a) and (e) indicate different azimuths ($0^\circ$ is under the transmitter wire, $90^\circ$ is orthogonal to it, and $180^\circ$ is opposite to it). The black line indicates the scenario for a well with permeability equal to that of free space $\mu_0$ and the red lines are for the scenario where the well has a permeability of $150\mu_0$. Panels (b), (c), and (d) show the ratio of the amplitude of the electric field with respect to the non-permeable well ($\mu=\mu_0$) for the test volume centered at a depth of 100m. Panels (f), (g) and (h) show the ratios of the electric field amplitude for the test volume centered at 400m depth.
}
\label{fig:excitation-time}
\end{figure}





==> figures/magnetization-currents-casing-freq-imag.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=0.8\textwidth]{figures/magnetization-currents-casing-freq-imag.png}
    \end{center}
\caption{
    Imaginary part of the components of equation \ref{eq:permeability-ampere-no-source-freq} at different frequencies.
}
\label{fig:magnetization-currents-casing-freq-imag}
\end{figure}





==> figures/magnetization-currents-casing-freq-real.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=\textwidth]{figures/magnetization-currents-casing-freq-real.png}
    \end{center}
\caption{
    Components of equation \ref{eq:permeability-ampere-no-source-freq} at different frequencies. Panels (a), (c), and (e) show the DC component of each term while (b), (d) and (f) show the inductive part of the real component (real - DC).
}
\label{fig:magnetization-currents-casing-freq-real}
\end{figure}





==> figures/magnetization-currents-casing.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=\textwidth]{figures/magnetization-currents-casing.png}
    \end{center}
\caption{
    Components of equation \ref{eq:permeability-ampere-no-source} through time: (a) the inductive term ($\mu\sigma\vec{e}$), (b) the magnetization term ($\nabla \ln \mu_r \times \vec{b}$), (c) curl of the magnetic flux ($\nabla \times \vec{b}$).
}
\label{fig:magnetization-currents-casing}
\end{figure}





==> figures/motivation-e-fields.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=\textwidth]{figures/motivation-e-fields.png}
    \end{center}
\caption{
    (a) Amplitude of the radial electric field 100m from the well.
    (b) Difference between the radial electric field amplitude for permeable and non-permeable wells.
    (c) Difference in the radial electric field as a percentage.
}
\label{fig:motivation-e-fields}
\end{figure}




